Wavelet-based parallel dynamic mesh adaptation for magnetohydrodynamics in the AMROC framework

Computational magnetohydrodynamics (MHD) for space physics has become an essential area in understanding the multiscale dynamics of geophysical and astrophysical plasma processes, partially motivated by the lack of space data. Full MHD simulations are typically very demanding and may require substantial computational efforts. In particular, computational space-weather forecasting is an essential long-term goal in this area, motivated for instance by the needs of modern satellite communication technology. We present a new feature of a recently developed compressible two- and three-dimensional MHD solver, which has been successfully implemented into the parallel AMROC (Adaptive Mesh Refinement in Object-oriented C++) framework with improvements concerning the mesh adaptation criteria based on wavelet techniques. The developments are related to computational efficiency while controlling the precision using dynamically adapted meshes in space-time in a fully parallel context.

==> graph.tex <==

\begin{figure}[htb]
\begin{center}
\resizebox{\textwidth}{!}{% <------ Don't forget this %
\begin{tikzpicture}[domain=-25:1,
declare function={ myf(\x,\xm) = (\x < \xm) * min{(max({\salf + (\a*(\x-\xm)/\xm)},0),1)} + !(\x <= \xm) * 0;
%\ifthenelse{\x < \xm}{max{(min({\salf + (\a*(\x-\xm)/\xm)},1),0)}}{0}];
                 },
]
      \def\xMin{-25}
      \def\yMin{-1}
      \def\xMax{1}
      \def\yMax{1}
      \foreach \i in {\xMin,...,\xMax} {
        \draw [very thin,gray] (\i,\yMin) -- (\i,\yMax)  node [below] at (\i,\yMin) {$\i$};
    }
    \foreach \i in {\yMin,...,\yMax} {
        \draw [very thin,gray] (\xMin,\i) -- (\xMax,\i) node [left] at (\xMin,\i) {$\i$};
    }
     \def\alf{10.0}
     \def\bet{1.2}
     \def\salf{1/sqrt{\alf}}
     \def\r{0.0005}
     \def\vsw{0.044}
     \def\xm{-16.6}
     \def\a{(1-\salf)/((\bet-1))}
     \draw[->,thick] (-25,0) -- (2,0) node[right] {{\large$x_{(\text{RE})}$}};
      \draw[->,thick] (0,-1.1) -- (0,1.1) node[above] {{\large$y_{(\text{RE})}$}};
  %  \draw[variable=\x,blue, very thick] plot ({\x}, {[\ifthenelse{\x < \xm}{max{(min({\salf + (\a*(\x-\xm)/\xm)},1),0)}}{0}]});
  \draw[variable=\x,blue, very thick] plot ({\x}, {myf(\x,\xm)});
  
  \node[below=0.2cm] at (-16.565038124,0) {$x_m$};
   \node[left=0.2cm] at (-25,0) {\Sun};
   \node[left=0.1cm,above=0.1cm] at (0,0) {\earth};
\end{tikzpicture}}
\end{center}
\caption{
An example of the IMF influence function $f(x,x_m)$ is drawn. It considers typical the parameters $\alpha=10$, $\beta=1.2$, $\rho_\text{sw}=5\cdot 10^{-4}$, $v_\text{sw}=0.044$, $B_0=1$,  $x_m=-16.57$.  
}
\end{figure}




\begin{table}[htb]
\caption{Solar wind parameters}
\resizebox{\textwidth}{!}{
\begin{tabular}{llllllllll}
\toprule 
\multicolumn{5}{l}{Solar wind (sw)} &
\multicolumn{3}{l}{IMF} \\
%
$\rho$ &
$p$ &
$v_{x}$ &
$v_{y}$ &
$v_{z}$ &
$B_{x}$ &
$B_{y}$ &
$B_{z}$ \\
\midrule
$5\cdot 10^{-4}$ &
$3.56\cdot 10^{-8}$ &
$4.4\cdot 10^{-2}$ &
$0.0$ &
$0.0$ &
$0.0$ &
$0.0$ &
$1.5\cdot 10^{-4}$\\
\bottomrule
\end{tabular}}
\end{table}




\begin{table}[htb]
\caption{Other parameters}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
$p_{00}$ &
$g_0$ &
$B_{0}$ &
$B_{s}$ &
$\alpha$ &
$\beta$ &
$ \text{RE}$ &
$\eta_0$ &
$\gamma$\\ \midrule
%units
$ $ &
$ $ &
$\langle \text{T}\rangle$  &
$ $ &
$ $ &
$ $ &
$ $ &
$ $  &
$ $ \\ \midrule
% data
$ $ &
$1.35$ &
$1$ &
$3.12\cdot 10^{-5}$ &
$10$ &
$1.2$ &
$0.0$ &
$0.01$ &
$\frac{5}{3}$\\
\end{tabular}}
\end{table}

%\url{https://tex.stackexchange.com/questions/130802/fill-a-contour-plot}

\[
\eta = \eta_0 \left[ \frac{T}{T_0} \right]^{-\frac{3}{2}}
\]

